Bayes Linear Emulation of Simulator Networks

Computationally expensive simulators, implementing mathematical models in computer codes, are commonly approximated using statistical emulators. We develop and assess novel emulation methods for systems best modelled via a chain, series or network of simulators. Using a Bayes linear framework, we link statistical emulators of the component simulators to explicitly account for the simulator input uncertainty induced by links between models in arbitrarily large networks. We demonstrate the advantages of these methods compared to use of a single emulator of the composite simulator network for a variety of examples, including the motivating epidemiological simulator chain to model the impact of an airborne infectious disease.

==> Arxiv version 2/Definitions.tex <==
%%% List of Definitions %%%

% Begin and end equations, lists, figures etc.
\newcommand{\be}{\begin{equation}}
\newcommand{\ee}{\end{equation}}
\newcommand{\ba}{\begin{eqnarray}}
\newcommand{\ea}{\end{eqnarray}}
\newcommand{\bi}{\begin{itemize}}
\newcommand{\ei}{\end{itemize}}
\newcommand{\bn}{\begin{enumerate}}
\newcommand{\en}{\end{enumerate}}
\newcommand{\bfi}{\begin{figure}}
\newcommand{\efi}{\end{figure}}

% Extended subfigure commands.
% subfig - file, prop. column width, scale, vertical space reduction to caption, caption, label, space underneath caption..
\newcommand{\subfig}[6]{\begin{subfigure}{#2\columnwidth}
\centering
\includegraphics[scale=#3]{#1}
\vspace{#4cm}
\caption{\footnotesize{#5}}
\label{#6}
\end{subfigure}}

% File where figures are stored.
\newcommand{\figfile}{R_Code_and_Figures/Figures}

% BL Expectations, variances etc.
\def \expectation  {\textrm{E}} 
\def \variance {\textrm{Var} }
\def \covariance {\textrm{Cov} }
\def \correlation {\textrm{Corr} }
\newcommand{\e}[1]{\ensuremath{{\rm E}[#1]}}
\newcommand{\ed}[2]{\ensuremath{{\rm E}_{#1}[#2]}}
\newcommand{\edhat}[2]{\ensuremath{{\hat{\rm E}}_{#1}[#2]}}
\newcommand{\var}[1]{\ensuremath{{\rm Var}[#1]}}
\newcommand{\vard}[2]{\ensuremath{{\rm Var}_{#1}[#2]}}
\newcommand{\vardhat}[2]{\ensuremath{{\hat{\rm V}\rm{ar}}_{#1}[#2]}}
\newcommand{\corr}[2]{\ensuremath{{\rm Corr}\left[#1,#2\right]}}
\newcommand{\corrd}[3]{\ensuremath{{\rm Corr}_{#1}\left[#2,#3\right]}}
\newcommand{\cov}[2]{\ensuremath{{\rm Cov}\left[#1,#2\right]}}
\newcommand{\covd}[3]{\ensuremath{{\rm Cov}_{#1}\left[#2,#3\right]}}
\newcommand{\aed}[2]{\ensuremath{{\rm \hat{E}}_{#1}[#2]}}
\newcommand{\avard}[2]{\ensuremath{{\rm \hat{V}ar}_{#1}[#2]}}

% Specifically with F
\newcommand{\eF}[1]{\ed{\bF}{#1}}
\newcommand{\varF}[1]{\vard{\bF}{#1}}
\newcommand{\covF}[2]{\covd{\bF}{#1}{#2}}
\newcommand{\eFX}[1]{\ed{\bF \cup \bX}{#1}}
\newcommand{\varFX}[1]{\vard{\bF \cup \bX}{#1}}
\newcommand{\covFX}[2]{\covd{\bF \cup \bX}{#1}{#2}}

% Full Bayesian expectations, variances etc.
\def \fbexp { \mathbb{E} }
\def \fbvar { \mathbb{V}ar }
\def \fbcov { \mathbb{C}ov }

% Conventional notations.
\def \indicator { \mathbb{I} }
\def \identity { \boldsymbol{I} }
\def \independent {\perp\!\!\!\perp} 
\def \GP { \mathcal{GP} }
\def \normal { \mathcal{N} }
\def \real { \mathbb{R} }
\def \det {\textrm {det}}
\def \trace {\textrm {trace}}
\def \vect {\textrm {vec}}

% Ensure math mode.
\newcommand{\cm}[1]{\ensuremath{ { #1 }}}

% Greek letters.
\def \al { \alpha }

% Mathcal letters.
\newcommand{\ma}{\mathcal{A}}
\newcommand{\mb}{\mathcal{B}}
\newcommand{\md}{\mathcal{D}}
\newcommand{\mk}{\mathcal{K}}
\newcommand{\mx}{\mathcal{X}}
\newcommand{\mz}{\mathcal{Z}}

% Bold letters.
\def \bbe { \mathbf{b} }
\def \bc { \mathbf{c} }
\def \bd { \mathbf{d} }
\def \bof { \mathbf{f} }
\def \bg { \mathbf{g} }
\def \bh { \mathbf{h} }
\def \bk { \mathbf{k} }
\def \bt { \mathbf{t} }
\def \bu { \mathbf{u} }
\def \bv { \boldsymbol{v} }
\def \bw { \boldsymbol{w} }
\def \bx { \mathbf{x} }
\def \by { \mathbf{y} }
\def \bz { \mathbf{z} }
\def \bA { \mathbf{A} }
\def \bB { \boldsymbol{B} }
\def \bC { \boldsymbol{C} }
\def \bF { \mathbf{F} }
\def \bG { \boldsymbol{G} }
\def \bH { \mathbf{H} }
\def \bK { \mathbf{K} }
\def \bL { \mathbf{L} }
\def \bT { \mathbf{T} }
\def \bU { \mathbf{U} }
\def \bW { \boldsymbol{W} }
\def \bX { \mathbf{X} }
\def \bZ { \mathbf{Z} }
\def \bb { \bm{\beta} }
\def \bGa{ \bm{\Gamma} }
\def \bDe { \boldsymbol{\mathit{\Delta}} }
\def \bet { \eta }
\def \br { \bm{\rho} }
\def \Sig { \boldsymbol{\mathit{\Sigma}} }
\def \bth { \bm{\theta} }
\def \bxi { \xi }
\def \bTh { \boldsymbol{\mathit{\Theta}} }
\def \bO { \boldsymbol{\mathit{\Omega}} }
\def \bizero { \boldsymbol{\mathit{0}} }
\def \bzero { \mathbf{0} }
\def \mbX { \mathbb{ X } }
\def \mbZ { \mathbb{ Z } }

% Composite and component simulators and inputs/outputs.
\def \com { \bh }  % Composite simulator bold h.
\def \cin { \bz } % Composite simulator input bold z.
\def \cout { \by } % Composite simulator output bold y.
\def \comin { \com(\cin) } % Composite simulator with input.
\def \simr { \bof } % Component simulator bold f.
\def \siin { \bx } % Component simulator generic input bold x.
\def \simrin { \simr(\siin) } % Component simulator with input. 
\def \simri { \simr^i } 
\def \simrj { \simr^j }
\def \simrcin { \simr^1(\bz) } 
\def \bez { \bt^E(\bz) }
\def \bvz { \bt^V(\bz) }
\def \cx { \bc(\bx) }
\def \cxp { \bc(\bx') }
\def \fx { \simr(\bx) }
\def \fxp { \simr(\bx') }
\def \gx { \bg(\bx) }
\def \gxp { \bg(\bx') }
\def \ux { \bu(\bx) }
\def \uxp { \bu(\bx') }
\def \vx { \bv(\bx) }
\def \vxp { \bv(\bx') }
\def \wx { \bw(\bx) }
\def \wxp { \bw(\bx') }
\def \cX { \bc(\bX) }
\def \cXp { \bc(\bX') }
\def \fX { \simr(\bX) }
\def \fXp { \simr(\bX') }
\def \gX { \bg(\bX) }
\def \gXp { \bg(\bX') }
\def \uX { \bu(\bX) }
\def \uXp { \bu(\bX') }
\def \vX { \bv(\bX) }
\def \vXp { \bv(\bX') }
\def \wX { \bw(\bX) }
\def \wXp { \bw(\bX') }


% Dispersion and DDR
\def \disp { d }
\def \dr { \rho }
\def \ddr { h }
\def \zSM { z_{SM} }
\def \zWD { z_{WD} }
\def \zWS { z_{WS} }
\def \dispin { \disp( \cin ) }

% Definitions for ease-of-notation-change if need be.
\def \simulator { f }
\def \mean { \mu }
\def \cl { \theta }
\def \meanvec { \bm{ \mu } }
\def \varmat { \bm{ \nu } }
\def \dist { \pi }

% sequences
\newcommand{\seq}[2]{#1,\dots,#2}
\newcommand{\seqsub}[3]{\seq{#1_{#2}}{#1_{#3}}}
\newcommand{\seqsup}[3]{\seq{#1^{#2}}{#1^{#3}}}
\newcommand{\seqsupb}[3]{\seqsup{#1}{(#2)}{(#3)}}
\newcommand{\funseq}[4]{\seq{#1_{#3}(#2)}{#1_{#4}(#2)}}
\newcommand{\fundes}[4]{\seq{#1(#2^{(#3)})}{#1(#2^{(#4)})}}
\newcommand{\fundesT}[4]{\seq{#1(#2_{#3})^T}{#1(#2_{#4})^T}}
\newcommand{\fundesiT}[5]{\seq{#1(#2^{#3(#4)})^T}{#1(#2^{#3(#5)})^T}}

% nomenclature
\newcommand{\nom}[2]{\nomenclature{$ #1 $}{#2}}

% Bayes linear calculations
\def \bOi { \bO^{-1}  } % Omega inverse.
\def \bDi { \bDe^{-1} }
\def \eb { \ed{\bF}{\bb} } % adjusted expectation for beta.
\def \ebt { \ed{\bF}{\bb^T} } % adjusted expectation for beta.
\def \vb { \vard{\bF}{\bb} } % adjusted variance for beta. 
\def \ewX { \e{\wX} } % expectation of w(X)
\def \vwX { \var{\wX} } % variance of w(X)
\def \WDW { \bW \, \bDe \, \bW^T }
\def \WOW { \bW^T \, \bOi \, \bW }
\def \WO { \bW^T \, \bOi }
\def \DG { \bDi \bGa }
\def \bbgls { \hat{\bb}_{GLS} }
\def \GCG { \bG^T \, \bC^{-1} \, \bG }
\def \GC { \bG^T \, \bC^{-1} }
\def \IxG  { ( \identity_q \otimes \bG ) }
\def \IxGt { ( \identity_q \otimes \bG^T ) }
\def \SxC { ( \Sig \otimes \bC ) }
\def \wix { \bw_i(\bX) }
\def \wjx { \bw_j(\bX) }

% New line
\newcommand{\NL}{ \nonumber \\ &&  \,\,\,\,\,\, } 
\newcommand{\NLeq}{ \nonumber \\  &=&} 












































